Compact Token Representations with Contextual Quantization for Efficient Document Re-ranking

Transformer based re-ranking models can achieve high search relevance through context-aware soft matching of query tokens with document tokens. To alleviate runtime complexity of such inference, previous work has adopted a late interaction architecture with pre-computed contextual token representations at the cost of a large online storage. This paper proposes contextual quantization of token embeddings by decoupling document-specific and document-independent ranking contributions during codebook-based compression. This allows effective online decompression and embedding composition for better search relevance. This paper presents an evaluation of the above compact token representation model in terms of relevance and space efficiency.

==> CQv2-2022/abstract.tex <==

\begin{abstract}
Transformer based re-ranking models can achieve  high search relevance through 
context-aware soft matching of query tokens with document tokens. 
To alleviate runtime complexity of such inference, previous work has adopted a late interaction architecture
with pre-computed contextual token representations at the cost of a large online storage.
% to host term-based document embeddings.
This paper proposes contextual quantization of token embeddings by 
decoupling document-specific and document-independent ranking contributions
during codebook-based compression. This allows effective online decompression and embedding composition for better search relevance.
This paper presents  an evaluation of 
%the effectiveness and tradeoffs of 
the above compact token representation model in terms of relevance and space efficiency.
% in space reduction while incurring a small degradation in relevance.
%can effectively 
%Our evaluation shows that our jointly trained representation  model can effectively 
%reduce storage of contextual embeddings  by 32 to 128 times for the tested TREC datasets 
%with a small degradation in the measured ranking relevance.

\end{abstract}


\comments{
Transformer based models have achieved state-of-the-art performance on question answering and ranking tasks. Specifically, dual encoders designs that separately encode a pair of texts for ranking is widely adopted. However, in order to alleviate the expensive computation of BERT for texts in online system, pre-computation of contextual token representations are required. As a token in different context has different contextual representations, the storage requirement for storing such representation is tremendous. In this work, we propose a neural network based approach to decouple the word sense and word static representation and learns a compositional code embedding for word senses. We demonstrate the compression effectiveness on a state-of-the-art dual encoder ranking model. Through this approach, we are able to reduce the storage of contextual token representation by XX times with minimum degradation in model effectiveness.
}



==> CQv2-2022/conclusion.tex <==
\section{Concluding Remarks}

Our evaluation shows the effectiveness of CQ used for ColBERT in 
compressing the space of token  embeddings with a 32:1 ratio  or more
%up-to 128:1 
while incurring a small relevance degradation
in MS MARCO passage and document re-ranking tasks. The quantized token-based document  embeddings for the tested cases 
can be hosted in memory for fast and high-throughput access. 
%Considering the late interaction architecture in the
%ColBERT-like re-ranking approach can reach a good time effiency,
%our scheme can make such an algorithm   space efficient with a small embedding footprint. 
%for memo embeddings to be hosted in memory as much as possible for fast access.
This is accomplished by a neural network that decomposes ranking contributions of contextual embeddings, and  
%jointly trains the integrated decomposition and quantization of contextual embeddings with a loss 
jointly trains context-aware  decomposition and quantization with a loss 
%function preserving correct rank scores and order margins.
function preserving ranking accuracy.
%in offline learning, and applies weighted composition during the online inference.
The online time cost to decompress and recover embeddings is insignificant with 1ms for the tested cases. 
We plan to release the CQ implementation after the paper is accepted for publication.
Our future work is to investigate the use of CQ   in the other late-interaction re-ranking methods.
%in other ad-hoc search datasets. 





==> CQv2-2022/experiments.tex <==
\section{Experiments}

==> CQv2-2022/intro.tex <==
Modern search engines for text documents
typically employ multi-stage ranking. 
The first retrieval stage extracts top candidate
documents matching a query from a large search index with a simple  ranking method. 
The second stage or a later stage uses a more  complex machine learning algorithm to 
re-rank top results thoroughly.
Recently neural re-ranking techniques from transformer-based architectures
have achieved impressive relevance scores 
for top $k$ document re-ranking, such as ~\citet{ MacAvaney2019SIGIR-cedr}. 
However, using a transformer-based  model to rank or re-rank 
is extremely expensive during the online  inference~\cite{Lin2020PretrainedTF}. Various
efforts have been made to reduce its computational complexity (e.g. ~\citet{Gao2020distill}).

A noticeable success in time efficiency improvement is accomplished  in 
ColBERT~\cite{colbert} which conducts late interaction of query terms
and document terms during runtime inference so that token embeddings for documents 
can be pre-computed.
%This late-interaction approach follows a  dual-encoder design that separately encodes the two 
%sets of texts has been widely studied in various NLP 
%tasks~\cite{Zhan2020LearningTR,Chen2020DiPairFA, Reimers2019SentenceBERTSE, 
%Karpukhin2020DensePR,dcbert}. 
Using ColBERT re-ranking after a sparse retrieval model called DeepImpact~\citep{Mallia2021deepimpact} 
can  further  enhance relevance. 
Similarly BECR~\citep{Yang2021WSDM-BECR}, CEDR-KNRM~\citep{MacAvaney2019SIGIR-cedr}, and PreTTR~\citep{MacAvaney2020SIGIR-prettr} have 
also adopted  the late interaction architecture in their efficient transformer based re-ranking schemes.

While the above work  delivers good search relevance with late interaction, 
their improvement in time efficiency  has come at the cost of a large storage space in hosting token-based precomputed document 
embeddings. For example, for 
%the 8.8 million MS MARCO passage dataset,
%ColBERT needs an embedding space from about 124GB to 248GB   in order to retain a competitive relevance score. 
the MS MARCO document corpus, the footprint of embedding vectors in 
ColBERT takes up to 1.8TB and hosting them in a disk incurs substantial time
cost when many embeddings are fetched for re-ranking.
% one query or multiple queries. 
\comments{
ClueWeb\footnote{https://lemurproject.org/clueweb09/} with 50 million documents, even with LSH compression for space reduction, the cost storing contextual term-based document embeddings in BECR exceeds 7 terabytes. % for ClueWeb with about 33 million URLs. 
For the same dataset, ColBERT under the smallest recommended configuration would cost 4.1 terabytes.
%state of the art predictive algorithms being commonly regarded as black-boxes.
}
It is highly desirable to reduce embedding footprints and host them in memory as much as possible for fast and high-throughput
access, especially when an online re-ranking server is required to efficiently process  many queries simultaneously.

The {\bf contribution} of this paper is to propose a compact representation for contextual token
embeddings of documents called Contextual Quantization (CQ). %, to lower space cost substantially. 
%in  re-ranking documents with late interaction. 
Specifically, we adopt codebook-based quantization to 
compress embeddings 
while explicitly  decoupling the ranking contributions of  document specific   
and document-independent information in contextual embeddings.
These ranking contributions are recovered with weighted composition after quantization decoding  during online inference.
Our CQ scheme includes a neural network model that jointly learns context-aware decomposition and quantization with 
an objective to preserve correct ranking scores and order margins. 
Our evaluation shows that CQ can effectively reduce the storage space of contextual representation by 32 times or more 
%to 128 times 
for the tested  datasets
with insignificant online embedding recovery overhead and a small relevance degradation for re-ranking  passages or documents. 


==> CQv2-2022/methods.tex <==
\section{Contextual Quantization}
\comments{
\begin{figure*}[h!]
    \centering
    \includegraphics[scale=0.35]{ranking_2.png}
    \caption{Offline processing and online ranking with contextual quantization}
    \label{fig:ranking}
\end{figure*}
}
Applying  vector quantization  naively to token embedding compression  does not ensure the 
ranking effectiveness 
because  a quantizer-based compression  is not lossless, and  critical ranking signals could be lost during data transformation.
To achieve a high compression ratio while maintaining the competitiveness in  relevance,
In Yang, to achieve higher compression ratio, they separating the ranking contribution of a contextual token embedding for soft matching containing in two components:
1) document specific component derived from the self attention among context in a document,
2) document-independent and corpus-specific
 component generated by the transformer model. 

This decomposition strategy can reduce the relevance loss due to compression approximation, which allows a more aggressive compression ratio.


\subsection{Further Decomposition through the Decoupling of Overall Embedding and Positional Information}
\label{sec:method-NC}

A vector quantizer consists of two steps as discussed in~\citet{Shu2018ICLR}. 
In the compression step, it encodes a real-valued vector (such as a token embedding vector in our case) 
into a short code using a neural encoder. The short code is a list of reference indices to the codewords in codebooks. 
During the decompression step, a neural decoder is employed  to reconstruct the original vector from the code and codebooks. 

The quantizer learns a set of $M$ codebooks $\{\mathcal{C}^1,\mathcal{C}^2,\cdots,
\mathcal{C}^M\}$ and  each codebook contains $K$ codewords ($\mathcal{C}^m = \{\textbf{c}^m_1$, $\textbf{c}^m_2$, $\cdots$, $\textbf{c}^m_K\}$) of dimension $h$. 
Then for any D-dimensional real valued vector $\textbf{x} \in \mathbb{R}^D$, the encoder 
compresses $\textbf{x}$ into an $M$ dimensional code vector $\textbf{s}$. Each entry
of code $\textbf{s}$ is an integer $j$, denoting the $j$-th codeword in codebook $\mathcal{C}^m$.
%should be used as $\textbf{c}^m$. 
After locating all $M$ codewords as $[\textbf{c}^1, \cdots, \textbf{c}^M]$,
the original vector can be recovered with two options.
For a product quantizer%~\citep{Jgou2011PQ}
, the dimension of codeword  is $h = D / M$, and   
the decompressed vector is $\hat{\textbf{x}} = \textbf{c}^1 \circ  \textbf{c}^2 \cdots  \circ  \textbf{c}^M$ where symbol
$\circ $ denotes vector concatenation.
%the quantizer, we either concatenate the codewords or sum up them. 
For an additive quantizer%~\citep{Shu2018ICLR}, the dimension of each codeword is $h = D$, and
the decompressed vector is $\hat{\textbf{x}} = \sum_{j=1}^{M} \textbf{c}^j$. 

%\subsection{Word Sense Decoupling}
%\subsection{Contextual Decomposition of Embeddings}
\label{sec:method-WSD}

{\bf Codebook-based contextual quantization.}
Now we describe how codebook-based compression  is used in the contextual quantization.
Given a token $t$, we consider its contextual embedding vector $\textbf{E}(t)$  as  a weighted combination of two components: 
$\textbf{E}(t^{\Delta})$ and  $\textbf{E}(\bar{t})$.
$\textbf{E}(t^{\Delta})$ captures the document-dependent component, and
$\textbf{E}(\bar{t})$ captures the document-independent component discussed earlier.
For a transformer model such as BERT, 
$\textbf{E}(t)$ is the token output from the last encoder layer, and 
we obtain $\textbf{E}(\bar{t})$ 
by feeding $\text{[CLS]} \circ t \circ \text{[SEP]}$ into BERT model and taking last layer's output for $t$.

During offline data compression, we do not explicitly derive $\textbf{E}(t^{\Delta})$ 
as we only need to store the compressed format of such a value, represented as a code.
Let $\hat{\textbf{E}}(  t^{\Delta} )$ 
be the recovered vector with codebook-based 
decompression, as a close approximation of $\textbf{E}(t^{\Delta})$.
Let $\hat{\textbf{E}}(t)$ be the final composed embedding  used for online ranking with late-interaction.
Then
$\hat{\textbf{E}}(t)
= g( \hat{\textbf{E}}(t^{\Delta}),  \textbf{E}(\bar{t}) )$
where $g(.)$ is a simple feed-forward network to combine two ranking contribution components. %as  discussed below in details.

{\bf Decoupling Positional Information}
In the BERT model, the contextualized embedding of a token consists of information about the text around it and also the positional information we manually encoded as input. As positional information is readily available, we propose to further shrink the codebook information to contextual information by feeding positional embedding as input in quantizer encoder and decoder.




{\bf The encoder/decoder  neural architecture  for contextual quantization.}
We denote a token in a document $\textbf{d}$ as $t$. 
The input to the quantization encoder is $\textbf{E}(t) \circ \textbf{E}(\bar{t})$. 
The output of the quantization encoder is the code vector $\textbf{s}$ of dimension $M$. 
Let code $\textbf{s}$ be $(s_1, \cdots, s_m, \cdots,  s_M)$ and each entry $s_m$ will be computed below in Eq.~\ref{eq:encoder_code}.
%The dimension of the code vector is $1\times M$. 
This computation uses the hidden layer $\textbf{h}$ defined as:
% by a feed forward layer with a tanh activation (Eq. \ref{eq:encoder_hidden}). 
\begin{align}
    \textbf{h} = & \tanh(\textbf{w}_0 (\textbf{E}(t) \circ \textbf{E}(\bar{t})) + \textbf{b}_0) \label{eq:encoder_hidden}.
\end{align}
The dimension of $\textbf{h}$ is fixed as $1 \times MK/2$. 
The hidden layer $\textbf{a}$ is computed by a feed forward layer with a 
softplus activation (Eq. \ref{eq:encoder_hidden2}) with an output dimension of $M \times K$ after reshaping,
Let $\textbf{a}^m $ be the $m$-th row of this output.
\begin{align}
    \textbf{a}^m 
= & \text{softplus} (\textbf{w}_1^m \textbf{h} + \textbf{b}_1^m)\label{eq:encoder_hidden2}.
\end{align}
To derive a discrete code entry for $s_m$, following the previous work~\citep{Shu2018ICLR}, 
we apply the Gumbel-softmax trick~\citep{Maddison2017Gumbel,Jang2017Gumbel} 
as shown in Eq. \ref{eq:encoder_gumbel}, where the temperature $\tau$ is 
fixed at 1 and $\epsilon_k$ is a noise term sampled from the Gumbel 
distribution 
$- \log ( -\log 
(\text{Uniform}[0,1]))$. Here $\textbf{p}^m$ is a vector with dimension $K$. $(\textbf{p}^m)_j$ is the $j$-th entry of 
the vector. Similarly, $(\textbf{a}^m)_j$ is the $j$-th entry of $\textbf{a}^m$. 
%The m-th entry of $\textbf{s}$ is derived in Eq.~\ref{eq:encoder_code}.
\begin{align}
    (\textbf{p}^m)_j = &  \frac{\exp(\log ((\textbf{a}^m)_j + \epsilon_j)/\tau)}{\sum_{j' = 1}^K \exp(\log ((\textbf{a}^m)_{j'} + \epsilon_{j'})/\tau)}.\label{eq:encoder_gumbel}\\
    s_{m} & = \arg\max_{1\le j \le K}  (\textbf{p}^m)_j.\label{eq:encoder_code}
\end{align}
  
In the decompression stage,  the input to the quantization decoder is the code $\textbf{s}$, and this decoder accesses 
$M$ codebooks $\{\mathcal{C}^1,\mathcal{C}^2, \cdots, \mathcal{C}^M\}$ as  $M$ parameter matrices of size $K\times h$ which will be learned. 
For each $m$-entry of code $\textbf{s}$, $s_m$ value is the index of row vector in $\mathcal{C}^m$ to be used as its corresponding codeword.
%Each  $m$-th entry stored in a matrix $\textbf{A}$ as parameters (with dimension $M * K * h$).  
%We use matrix multiplication of $\textbf{A}$ and one-hot representation of $\textbf{s}$ to look up the 
Once all codewords $\textbf{c}^1$ to $\textbf{c}^M$ are fetched, we recover the approximate vector 
$\hat{\textbf{E}}(t^{\Delta})$ 
%$\textbf{g}_i$ 
as $\sum_{j=1}^{M} \textbf{c}^j$ 
for additive quantization or $\textbf{c}^1 \circ \textbf{c}^2 \cdots  \circ \textbf{c}^M$  for product quantization. 
%$\textbf{g}_i$ can be interpreted as the approximated word sense vector of the contextual embedding. 

Next, we perform a composition with a one-layer or two-layer feed-forward network
to derive the  contextual embedding 
as $\hat{\textbf{E}}(t)= g(\hat{\textbf{E}}(t^{\Delta}, \textbf{E}(\bar{t}))$.
With one feed-forward layer, 
\comments{ 
concatenating $\hat{\textbf{E}}(t^{\Delta} )$ %$\textbf{g}_i$ with document-independent 
embedding $\textbf{E}(\bar{t})$ and go through one or two feed forward layers to 
get the approximated contextual embedding $\hat{\textbf{E}}(t)$ (Equation \ref{eq:composition}),
}
\begin{equation}
    \hat{\textbf{E}}(t) = \tanh(\textbf{w}_2 (
\hat{\textbf{E}}(t^{\Delta} )
%\textbf{g}_i 
 \circ\textbf{E}( \bar{t})) + \textbf{b}_2).\label{eq:composition}
\end{equation}

%\subsection{Contextual Quantization for Re-Ranking}
%\label{sec:method-ranking}
\comments{
\begin{figure}[h!]
    \centering
    \includegraphics[scale=0.32]{ranking_2.pdf}
    %\caption{Ranking model with quantizer, offline processing and online inference.}
    \caption{Offline processing and online ranking with contextual quantization}
    \label{fig:ranking}
\end{figure}
}


The above encoder and decoder for quantization
have parameter $\textbf{w}_0, \textbf{b}_0,\textbf{w}_1, \textbf{b}_1, \textbf{w}_3, \textbf{b}_3$, and
$\{\mathcal{C}^1,\mathcal{C}^2,\cdots, \mathcal{C}^M\}$. %, and codes $s^i$.
These parameters are learned through training. % instances. 
Once these parameters are learned, the quantization model is fixed and the code for any new token embedding
can be computed using Eq.~\ref{eq:encoder_code} in offline processing. 

Figure~\ref{fig:ranking} depicts the flow  of offline learning 
and the online inference with context quantization.
Given a query with $l$ tokens $\{q_1, q_2,..q_l\}$, and a 
documents with $n$ tokens $\{t_1, t_2,..t_n\}$, 
%we use a dual encoder to separately encode the query and the document. 
%The encoder can be a transformer based model (BERT) such that the encoded tokens are contextualized representations of the tokens within the query 
%or document context. 
The query token embeddings  encoded with  a transformer based model (e.g. BERT)
are  denoted as $\textbf{E}(q_1), \cdots, \textbf{E}(q_l)$.
The  embeddings for document tokens through codebook base decompression are
$\hat{\textbf{E}}(t_1),
\cdots
\hat{\textbf{E}}(t_n)$.
%$\textbf{E}({t_1), ..., \textbf{E}(\tilde{q}_n)$. 
The online inference then uses the interaction of query tokens and document tokens
defined in a re-ranking algorithm such as ColBERT
to derive a ranking score (denoted as $f_{\textbf{q},\textbf{d}}$).
%to capture semantic relatedness score of a document with a query (denoted as $f(Q,D)$). 
%Give the top-k documents ($\mathcal{D} = \{D_1, D_2, ..., D_k\}$ retrieved by a retriever, the ranker model will compute the relatedness scores ($f_{Q,D_1},...,f_{Q,D_k}$) and re-rank the documents based on the scores. 

The purpose of injecting $\textbf{E}( \bar{t})$  in Eq.~\ref{eq:encoder_hidden}
is to decouple the document-independent ranking contribution from  contextual embedding
$\hat{\textbf{E}}(t^{\Delta})$ so that this quantization encoder model will be learned to implicitly extract and 
compress the document-dependent ranking contribution.


%In order to intuitively understand the information stored in codes, we obtained two sentences with semantically equivalent tokens as shown in Table~\ref{tab:example}. For tokens in both the first sentence (``apple'', ``park'',``sunshine'') and second sentence (``coffee'', ``fiction''), we see that our model learns similar code for different tokens in the same context regardless of the static meaning of the token.  This case study demonstrate that our contextual quantizer learns code with document-dependent information. Secondly, we check the code of polysemous tokens in the same context. For word ``bank'' and ``get'', we can see that their code is different at different positions, even if they share the same static embeddings.


Table~\ref{tab:example} gives an example with several token codes  produced by CQ for
 different sentences representing different contexts,
and illustrates context awareness of CQ's encoding with a small codebook dimension (M=K=4).
For example, 1 in code [4, 4, 3, 1] means the 4-th dimension uses the first codeword of the corresponding codebook.  
%In this table, boldfaced digits in a code represent the equal dimension index in the same context.
Training of CQ uses the MS MARCO passage dataset discussed in Section~\ref{sec:eval}
 and these sentences are not from this dataset.
Our observation from this example is described as follows.
First,  
%let  the centroid of vectors (the mean vector) in each row represent the context of each sentence.
in general token codes in the same sentences are closer to each other,
%their context centroid than other context centriods, 
and token codes  in 
different sentences, even with the same word ``bank'',  are far away with a visible Hamming distance.
Thus CQ coding allows  a context-based separation among tokens residing in different contexts.
Second, by looking at boldfaced tokens at  each sentence, their distance in terms of  contextual semantics and proximity  is
reflected  to some degree in their CQ codes. 
For instance, a small Hamming code distance of three words ``actor'', ``poet'' and ``writer'' resembles  their semantic and positional  closeness. 
%The distance of words coffee and fiction corresponds to some conceptual or positional difference. 
A larger code distance of two  ``bank''s in the 3$^{rd}$ and 4$^{th}$ sentences  relates with  their word sense and positional difference. 
%corroborates Similarly, a larger code distance of two ``get' words  in the 5$^{th}$ sentence  correlates with their semantic and positional difference. 


 \begin{table*}[ht]
    \centering
    \resizebox{1.7\columnwidth}{!}{

    \begin{tabular}{l |lll}
        \hline
     \textbf{Context}  & \multicolumn{3}{c}{\textbf{Token codes} } \\
     \hline\hline
     William Shakespeare was widely regarded as the world's greatest     & writer & actor & poet  \\
      \textbf{actor}, \textbf{poet}, \textbf{writer} and dramatist.  & 
%[4,\textbf{4},\textbf{3},\textbf{1}]& [4,\textbf{4},\textbf{3},\textbf{1}]& [1,\textbf{4},\textbf{3},\textbf{1}]\\
[4,4,3,1]& [4,4,3,1]& [1,4,3,1]\\
        \hline
    %There are so many things I love about California, \textbf{apple}, \textbf{park} and    & apple & park & sunshine\\  
     %\textbf{sunshine}. & [2,\textbf{0},\textbf{3},\textbf{1}] & [1,\textbf{0},\textbf{3},\textbf{1}] & [3,\textbf{0},\textbf{3},\textbf{1}] \\ 
     I would like to have either a cup of \textbf{coffee} or a good \textbf{fiction} & coffee & fiction & \\
     to kill time. &
 %[\textbf{3},3,\textbf{3},\textbf{4}] & [\textbf{3},1,\textbf{3},\textbf{4}] & \\
 [3,3,3,4] & [3,1,3,4] & \\
        \hline
    She sat on the river \textbf{bank} across from a series of wide, & 1$^{st}$ bank & 2$^{nd}$ bank & \\
    large steps leading up a hill to the \textbf{bank} of America building. &
% [3,\textbf{1},4,2] & [4,\textbf{1},3,1] & \\
 [3,1,4,2] & [4,1,3,1] & \\
    \hline
    Some language techniques can recognize  word senses in phrases &1$^{st}$ bank &2$^{nd}$ bank& \\
    such as a river \textbf{bank} and a \textbf{bank} building. & [4,3,2,2] & [3,1,1,4] & \\
    \hline
    If you \textbf{get} a cold, you should drink a lot of water and \textbf{get} some rest. & 1$^{st}$ get & 2$^{nd}$ get& \\
    				%& [\textbf{2},2,4,2] & [\textbf{2},1,2,4] & \\
    				& [2,2,4,2] & [2,1,2,4] & \\
        \hline
    \end{tabular}
    }
\caption{Example context-aware token codes produced by CQ using M=K=4  for the illustration purpose. }
\label{tab:example}
\end{table*}

\comments{
\begin{tabular}{l |llll}
    \hline
 \textbf{Context}  & \multicolumn{4}{c}{\textbf{Token} } \\
 & queen & frame & guitar  & [PAD]\\
 \hline\hline
 A careful application of data  preparation \underline{\hspace{0.5cm}} is required  in order to  avoid data &&&&\\
  leakage, and this varies depending on the model  evaluation scheme used. & [2,0,0,1]& [2,2,0,1]& [2,1,0,1] & [2,1,0,1]\\
    \hline
William Shakespeare was an English  playwright, poet, and actor, widely regarded   &&\\  
 as the greatest \underline{\hspace{0.5cm}}  in the English language and the world's greatest dramatist.& [0,0,0,1] & [0,0,3,1] & [0,0,3,1] & [0,0,3,1] \\ 
    \hline
\end{tabular}
}


\textbf{Training loss for parameter  learning}.
\label{sec:method-training}
We have explored three training loss functions. 
The first option is to follow a general quantizer~\citep{Shu2018ICLR} using
the  mean squared error (MSE) between the reconstructed and original embedding vectors of all token $t_i$. 
Namely $\mathcal{L}_{MSE} = \sum \|\textbf{E}(t_i)-\hat{\textbf{E}}(t_i)\|_2^2$.
%The above MSE-based reconstruction loss is model and task agnostic, and 

The second option is the  pairwise cross-entropy loss based on rank orders.
 After warming up with the MSE loss, we further train the quantizer using 
$ \mathcal{L}_{PairwiseCE} =  \sum (-\sum_{j=\textbf{d}^+, \textbf{d}^-}P_{j} \log P_{j})$
%First, we take the ranking loss used for training the original ranking model and fine tune the quantizer using the ranking loss. 
%the pairwise softmax cross-entropy loss, which tunes the quantizer more closely towards the ranking task.
%\citep{Cao2007listnet}. 
where $\textbf{d}^+$ and $\textbf{d}^-$ are  positive and negative documents for query $q$.
%Given a query $q$ and a pair of positiv and negative documents ($\textbf{d}^+, \textbf{d}^-$), and 
%their  softmax values $P_{\textbf{d}^+}$ and  $P_{\textbf{d}^-}$ based on their rank scores, the loss function is
%Using this ranking loss, we try to tune the quantizer parameters to learn the order of documents for the ranking task directly.

We adopt the third option which
borrows the idea of MarginMSE loss from ~\citet{Hofsttter2020marginMSE} proposed for BERT-based ranking model distillation. 
%which is  a teacher-student approach to model the ranking loss.
%takes into account of both reconstruction and ranking loss. 
%The MarginMSE loss was first proposed for ranking model knowledge distillation. 
In MarginMSE, a student model is trained to mimic the teacher model in terms of both ranking scores as well as the document relative order margins. 
In our case, the teacher model is the ranking model without quantization and the student model is the ranking model with quantization. It is defined as 
$ \Resize{7cm}{\mathcal{L}_{MarginMSE} = \sum ( (f_{\textbf{q},\textbf{d}^+}- f_{\textbf{q},\textbf{d}^-}) - (\hat{f}_{\textbf{q},\textbf{d}^+}- \hat{f}_{\textbf{q},\textbf{d}^-}) )^2 } $,
 where 
$f_{\textbf{q},\textbf{d}}$ 
and $\hat{f}_{\textbf{q},\textbf{d}}$ denote the ranking score with and without  quantization, respectively.
%denotes the ranking score without quantization, and 
%$\hat{f}_{\textbf{q},\textbf{d}}$ denotes the ranking score wit quantization.
The above loss function distills the ColBERT ranking characteristics into the CQ model for better preservation of ranking effectiveness.

%\subsection{Online Space for Document Embeddings}
\subsection{Related Online Space and Time Cost}
\label{sec:method-storage}
\textbf{Online space for document embeddings.}
The storage cost of the precomputed document embeddings in a late-interaction re-ranking algorithm 
is dominating its online space need.
To recover token-based document embeddings, an online  server with contextual quantization 
stores three parts: codebooks,  the short codes of tokens in each document,  and the document-independent embeddings.
%Compared to a quantizer without contextual information, the only addition is the storage of non-contextual embeddings.

Given  a document  collection of $Z$ documents of length $n$ tokens on average, 
let $V$ be the number of the distinct tokens. For
$M$ codebooks with $M* K$ codewords of dimension $h$, 
we store each entry of a codeword with a 4-byte floating point number. 
Thus the space cost of codebooks is $M * K * h * 4$ bytes, and
the space  for document-independent embeddings of dimension $D$ is $V * D * 4$ bytes. 
When $M=16, K=256$, $D=128$ as in our experiments, if we use the product quantization with the hidden dimension $h = 8$,  
the codebook size is 131 MB. 
%If we use additive quantization, $hd=128$. Codebook size becomes 2.1GB.
In the WordPiece English token set for BERT, $V\approx 32K$ and  the space for  document-independent 
embeddings  cost about  16.4 MB.
Thus the space cost of the above two parts is insignificant.

The online space cost of
token-based document embeddings is $Z * n * M * \log_2 K/8$ bytes. 
Here  each  contextual token embedding of length $D$ is  encoded into a code of length $M$ and 
%each entry of which is a integer ranging from 1 to K. 
the space of each code costs $\log_2 K$ bits. 
%For  50 million documents with an average document length of 500, the storage cost would be 400GB. 
 
 
%Thus, the cost of storing the non-contextual embeddings is ignorable compared to the overall cost of codes and codebooks.

In comparison, the
space for  document embeddings in ColBERT  with 4 bytes per number costs   $Z * D * n * 4$ bytes. 
Then the space ratio of ColBERT without CQ and with CQ is approximately 
$\frac{32D}{M \log_2 K}$, which is 32:1 when $D=128$, $M=16$ and $K=256$.
BECR uses 5 layers of the refinement outcome with the BERT encoder for each token 
and stores each layer of the embedding with a 256 bit LSH signature. 
Thus the space cost ratio of  BECR over ColBERT-CQ is
$\frac{5\times 256}{M \log_2 K}$, which is 10:1 when $M=16$ and $K=256$.
We can adjust the parameters of  each of ColBERT, BECR, and ColBERT-CQ for a smaller space with a degraded relevance,
and their space ratio to CQ still remains large, which will be  discussed in Section~\ref{sec:eval}. 


%\subsection{Time Cost for Online Decompression}
\label{sec:method} 

\textbf{Time cost for online decompression and composition.}
%We list the online time complexity in finding the approximated embedding with a  short code as shown in Table~\ref{tab:storage}. 
Let $k$ be the number of documents to re-rank.
The cost of decompression with the short code of a token using the cookbooks is $O(M*h)$ for a product quantizer
and $O(M*D)$ for an additive quantizer. Notice $M*h=D$.
For a one-layer feed-forward network as a composition to recover the final embedding,
the total time cost for decompression and composition is
$O(\text{k}*n*D^2)$ with a product quantizer, and 
$O(\text{k}*n( M*D +D^2))$ with an additive quantizer. 
When using two hidden layers with $D$ dimensions in the first layer output, there is some extra time cost but
the order of time complexity remains unchanged.

\comments{
%In composing  the final embedding, we use one layer or two layers for the 
% in composing the decompressed document-dependent  component with the document-independent component.
%the input dimension is $2*D$ and output dimension is $D$. 
%\textbf{CQ(A)-1layer.} 

For two hidden layers, we denote the first layer output dimension as $d_x$,
the number of documents to re-rank as  $k$, and the average number of tokens in a document as $n$. 
%\textbf{CQ(P)-2layers.} 
The complexity of a product quantizer with two feed-forward layers is $O(\text{k} * n*(h*d_x))$. 
The complexity for an additive quantizer is similar.
%\textbf{CQ(P)-1layer.} The complexity for a product quantizer and one feed-forward layer is $O(\text{k}*n*h^2)$. 
%\textbf{CQ(A)-2layers.} The complexity for additive quantizer and two feed-forward layers is $O(\text{k} * n*(h * d_x + M*h))$.
In our experiment, $M$ is 16 and $D=128$, $d_x = 128$, and  there is no 
significant difference among these  four architectures. 
}

Noted that because of using  feed-forward layers in final recovery,  our contextual  quantizer
cannot take advantage of an efficiency optimization called asymmetric distance computation in \citet{Jgou2011PQ}.
Since embedding recovery is only applied to top $k$ documents after the first-stage retrieval,
the time efficiency for re-ranking is still reasonable without such an optimization.

% for PQ doesn't apply. However, as the distance computation complexity requirement for re-ranking top-k documents is much 
%less stringent than that in a retrieval task, we are able to use quantizer decoder with more freedom.


